Robust Algorithms for the Secretary Problem

In classical secretary problems, a sequence of $n$ elements arrive in a uniformly random order, and we want to choose a single item, or a set of size $K$. The random order model allows us to escape from the strong lower bounds for the adversarial order setting, and excellent algorithms are known in this setting. However, one worrying aspect of these results is that the algorithms overfit to the model: they are not very robust. Indeed, if a few "outlier" arrivals are adversarially placed in the arrival sequence, the algorithms perform poorly. E.g., Dynkin's popular $1/e$-secretary algorithm fails with even a single adversarial arrival. We investigate a robust version of the secretary problem. In the Byzantine Secretary model, we have two kinds of elements: green (good) and red (rogue). The values of all elements are chosen by the adversary. The green elements arrive at times uniformly randomly drawn from $[0,1]$. The red elements, however, arrive at adversarially chosen times. Naturally, the algorithm does not see these colors: how well can it solve secretary problems? We give algorithms which get value comparable to the value of the optimal green set minus the largest green item. Specifically, we give an algorithm to pick $K$ elements that gets within $(1-\varepsilon)$ factor of the above benchmark, as long as $K \geq \mathrm{poly}(\varepsilon^{-1} \log n)$. We extend this to the knapsack secretary problem, for large knapsack size $K$. For the single-item case, an analogous benchmark is the value of the second-largest green item. For value-maximization, we give a $\mathrm{poly} \log^* n$-competitive algorithm, using a multi-layered bucketing scheme that adaptively refines our estimates of second-max over time. For probability-maximization, we show the existence of a good randomized algorithm, using the minimax principle.

==> missing_proofs.tex <==
% !TeX root = main.tex
% !TEX root = main.tex

\section{Missing Proofs} \label{sec:missingProofs}

\agnote{Keep or remove?}

%\obsSubSampling*
\begin{proof}[Proof of Observation~\ref{obsSubSampling}]
  We construct $\calA'$ in the following way. Run $\calA$ on the input and each time it selects an element $e$, we decide to select it in $\calA'$ with probability $\frac{r}{r'}$ or discard it otherwise. If at some point $\calA'$ selects $r$ items, we stop selecting new elements. 
  
Let $S$ be the set selected by $\calA$ (a random variable) and let $S'$ be the set of elements of $S$ independently subsampled with probability $\frac{r}{r'}$. Finally, let $S'' \defeq S'$ if $|S'| \le r$ and $S'' \defeq \emptyset$ otherwise. Note that by construction $v(\calA') \ge v(S'')$.

  Fix $S$ and consider the expected contribution $[e \in S'']v(e)$ of an element $e \in S$, here $[P]$ is the Iverson bracket.
  We have that
  \begin{align*}
    [e \in S'']v(e) \ge \frac{r}{2r'} \Pr[|S' \setminus \{e\}| < r] v(e) \ge \Pr[|S'| < r] v(e) .
  \end{align*}
  By Markov, $\Pr[|S'| \ge r] \le \E[|S'|] / r = (|S| \frac{r}{2r'}) / r = \frac{1}{2}$.
  Hence,
  \begin{align*}
    E[ALG' \mid S] \ge \sum_{e \in S''} \frac{r}{2r'} [e \in S'']v(e) \ge \frac{1}{2} \frac{r}{2r'} v(S).
  \end{align*}
  By assumption we have that $\E[v(\calA)] = \sum_{U \subseteq [n]} \Pr[S = U] v(S)$. Hence we have
  \begin{align*}
    \E[ALG'] \ge \sum_{U \subseteq [1\ldots n]} \Pr[S = U] \E[ALG' \mid S] \ge \sum_{U \subseteq [1\ldots n]} \Pr[S=U] \frac{r}{4r'} v(S) = \frac{r}{4 r'} E[v(\calA)] \ge \alpha \frac{r}{4 r'} V^*.
  \end{align*}
\end{proof}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "arxiv"
%%% End: 


==> uniform_matroid.tex <==
% !TeX root = main.tex 
% !TEX root = main.tex

\subsection{$O(1)$-approximation for Uniform Matroids}\label{sec:uniform-matroids-value}
Consider the $r$-uniform matroid setting, i.e, where we can select any $r$ elements. 
 Let $g_{\max}, g_2, g_3, \ldots, g_{r+1}$ denote the top $r+1$ green elements (pad with elements of zero value if necessary) and let $V^* = \sum_{i=2}^{r+1} v(g_i)$ be the benchmark solution after discarding the top green element. 
We show that for  $r = \Omega(\log n)$ there exists an $O(1)$ approximation.

\begin{restatable}{observation}{obsSubSampling}
  \label{obsSubSampling}
  Suppose we are given  an $r$-uniform matroid problem with a benchmark solution of value $V^*$ and an algorithm $\calA$ that selects at most $r' \ge r$ elements.  If $\E[v(\calA)] \ge \alpha V^*$ then we can transform $\calA$ into an algorithm $\calA'$ that selects at most $r$ elements and has value $\E[v(\calA')] \ge \alpha \frac{r}{4r'} V^*$.
\end{restatable}
The idea in the proof of Observation~\ref{obsSubSampling} is to run $\calA$ but select each element only w.p. $\frac{r}{r'}$ until we select $r$ elements. In Appendix~\ref{sec:missingProofs} we show every element of $\calA$ gets selected by $\calA'$ w.p. at least $1/4 \cdot r/r'$, which implies this observation. Hence,  to find an $O(1)$-approximation for an $r$-uniform matroid, it is sufficient to find a $O(1)$-approximation (with respect to the original benchmark solution) while selecting at most $r' \defeq r + \log n$ elements.

%\textbf{Algorithm for selecting $r' = r + \log n$ elements. }
\subsubsection{The Algorithm for Selecting $r'$ Items}
We define $r' + 1$ time \emph{checkpoints} as follows: the initial
checkpoint $\checkp_0 = \frac{1}{2}$, and then subsequent checkpoints
$\checkp_i = \frac{1}{2} + \frac{i}{2 r'}$ for all
$i \in [1\ldots r']$. 
Now the corresponding intervals are
\begin{gather}
  \I_0 \defeq [0, \checkp_0] \quad   \text{and}   \quad \I_i = \ocinter{ \checkp_{i-1},
  \checkp_i} \quad \forall \, i \in [1\ldots r'].
\end{gather}

%For conceptual convenience we first split the time into two parts: $\cointer{0, 1/2}$ and $\cointer{1/2, 1}$; then we partition the latter into $r'$ intervals $I_0, I_1, \ldots, I_{r'-1}$ where $\I_i = \cointer{1/2 + j\frac{1}{2r'}}$.
Our algorithm runs one of the following two algorithms chosen  uniformly at random.

\begin{enumerate}[label=(\roman*)]
\item Select an  element  uniformly at random as discussed in \S\ref{sec:two-useful}.  \label{alg:uniformOne}
\item Observe the largest value element $v_0$ in $\I_0$. Initialize a threshold $\tau$ to $\tau \gets \frac{v_0}{2 n r'}$ and perform the following during time $\ocinter{1/2, 1}$. Whenever we encounter an element $e$ with value $v(e) \ge \tau$, we increase $\tau$ to $\tau \gets 2 \tau$ and select $e$ (i.e., include it into our solution) unless we have already selected  $r'$ elements. Whenever we reach an end of an interval $\I_i$ for $i \in [1 \ldots r'] $, we decrease $\tau$ to $\tau \gets \frac{1}{2}\tau$. Finally, whenever $\tau$ falls below $\frac{v_0}{2nr'}$, set $\tau \gets \frac{v_0}{2nr'}$. \label{alg:uniformTwo}
\end{enumerate}

\subsubsection{The Analysis}
Suppose that any element in $R \cup G$ has value at least $n V^*$. Then Algorithm~\ref{alg:uniformOne} has an expected $\Omega(V^*)$ and we are done.  From now assume this is not the case. Moreover, we condition on the probability $1/2$ event that the largest green element $g_{\max}$ arrives in $\I_0$, which implies
\[ v(g_{\max}) \leq v_0 \leq  nV^*. \]


Let $G' \subseteq G$ denote the set of good (green) elements from the benchmark solution that satisfy the following three properties:
\setlist{nolistsep}
\begin{enumerate} [label=(\alph*),noitemsep]
\item Arrive  during time $\ocinter{1/2, 1}$.
\item Have value at least $\frac{v_0}{2 n r'}$.
\item In the interval $\I_i$ they arrive, have the highest value among the benchmark solution elements.

\end{enumerate}
We show that WLOG we can focus our attention only on the elements in $G'$.

\begin{claim}
$\E[v(G')] = \Omega(V^*)$.
\end{claim}
\begin{proof}
Since each green element has $1/2$ chance of appearing after $t=1/2$, we can assume the first property. For the second property, notice that the elements with value below $ \frac{V^*}{2 r'}$ can contribute at most $1/2 \cdot V^*$. Since $\frac{v_0}{2 n r'} \leq \frac{V^*}{2 r'}$, we can  assume the second property. 

Finally, for the third property, consider any element $g_j$ for $j \in [2\ldots r'+1]$ that appears in some interval $\I_i$, $i \in [1 \ldots r']$. The probability that no other benchmark solution element appears in this interval is at least  $(1 - \frac{1}{r'})^{r'-1} \ge 1/e$. Hence we can assume the third property.
\end{proof}


%Let $G'' \defeq \{ g \in G' \mid v(g) \ge \frac{V^*}{2 r'} \}$ be the elements in the optimal solution excluding ones with value below $\frac{V^*}{2r'}$.

%\begin{claim}  $v(G'') = \Omega(v(G'))$ \end{claim}
%\begin{proof}   We have that $v(G'') = v(G') - v(G' \setminus G'') = v(G') - \frac{V^*}{2 r'} \cdot r' = V^* - V^*/2 = V^*/2 $. \end{proof}

%???. Furthermore, since $v_0 < n V^*$, we have that $\frac{v_0}{2 nr'} < \frac{V^*}{2r'}$, hence discarding input elements below $\frac{v_0}{2 n r'}$ decreases the benchmark solution only by a constant.

%As a final reduction of the benchmark solution, let $G'''$ be the following: for all $\I_i, j \in \{0, \ldots, r'-1\}$ insert into $G'''$ only the highest value green element that landed during $\I_i$; continue to the next interval if no such element exists in $\I_i$.

%\begin{claim}   $\E[v(G''')] = \Omega(v(G''))$ \end{claim}
%\begin{proof}   Consider the following stochastic process and let $X \gets 0$. Let $v(e_1) \ge v(e_2) \ge \ldots \ge v(e_{|G''|})$ be the elements of $G''$ in order of nonincreasing values. Uniformly randomly assign $e_i$ to one of the intervals $I_{j(i)} \in \{I_0, \ldots, I_{r'-1}\}$. If $e_i$ is the first one being assigned to $J_{j(i)}$, insert it into the set $X$ and continue otherwise. It is clear that the distribution of $X$ and $G'''$ are the same. 

%  By the above process we have that $\Pr[e_i \in X]$ is equal to the expected fraction of empty intervals $\I_i$, which is exactly $(1 - \frac{1}{r'})^{i-1} \ge (1 - \frac{1}{r'})^{r'-1} \ge 1/e$. Hence we have that $\E[v(G''')] = \E[v(X)] = \sum_{e \in G''} \Pr[e \in X]v(e) \ge \frac{1}{e}v(G'')$, as required. \end{proof}


Let $S \subseteq R \cup G$ be the set of  elements selected by our algorithm. In the following lemma we show its value is comparable to $v(G')$.

\begin{lemma}
  $\E[v(S)] = \Omega(\E[v(G')])$.
\end{lemma}
\begin{proof}
  Let $X \defeq G' \setminus S$ denote the set of elements from $G'$ that are not selected by the algorithm. The claim is clearly true if $X = \emptyset$. For the missed  elements $e \in X$, which arrived at time $t_e$, we show how to ``charge'' its value to the latest  selected element that arrived before $e$, i.e.,  to $\arg\max_{s \in S, t_s < t_e}\{ t_s \}$.
    Notice that some element has been selected before $e$ because we initialize 
    \[ \tau = \frac{v_0}{2 n r'} \le \frac{V^*}{2 r'} \le v(e).\] 
    
    Our charging scheme defines a function $c : S \to \mathbb{R}_{\ge 0}$, where we say $c(s)$ is the amount charged to $s \in S$. We denote $c(E) = \sum_{e \in E} c(e)$ for any set $E \subseteq S$.  Since every element $x \in X$ was charged to exactly one $s \in S$, we have $v(X) = c(S)$.

  Fix a $s \in S$ and consider the set of elements $x_1, x_2, \ldots, x_k \in X$ that are charged to $s$ ordered by their time of arrival. For an element $e \in R \cup G$ let $\tau_e$ be the threshold value $\tau$ of the algorithm at the moment of arrival of $e$. Since $s \in S$  and $x_j \not \in S$ for $j \in [1\ldots k]$,   we have  $v(s) \geq \tau_s$ and   $v(x_j) < \tau_{x_j}$.

  By construction of $G'$, element $x_j$'s arrived in a distinct interval $\I_i$ and no element was chosen between $s$ and $x_j$. Hence, $\tau$ was only exponentially decreasing between $t_s$ and $t_{x_j}$. This means $\tau_{x_1} \le 2 \tau_s$ because after selecting $s$ the value of $\tau$ doubles and is decreasing;  $\tau_{x_2} \le \tau_s$ since there is an end of an interval $\I_i$ between $t_{x_1}$ and $t_{x_2}$, and $\tau$ halves at those checkpoints; and so on. We therefore have 
  \[ c(s) \quad = \quad \sum_{i=1}^k v(x_j) \quad < \quad \sum_{i=1}^k \tau_{x_j} \quad \le \quad \tau_s \sum_{i=1}^k \frac{4}{2^i} \quad  \le \quad 4 \tau_s \quad \le \quad 4 v(s),\]
   which implies $c(S) \le 4 v(S)$ by additivity. Moreover, $c(S) = v(X)$ implies $v(X) \le 4 v(S)$. 
   Finally, since $S \cup X \supseteq G'$, we conclude this lemma by
   \[ v(S) + 4 v(S) \quad \ge \quad v(S \cup X) \quad \ge \quad v(G') \quad = \quad V^* . \qedhere \] 
\end{proof}

Now to prove Theorem~\ref{thmUnif}, we combine Observation~\ref{obsSubSampling} with
 \[ \E[v(\calA)] \quad = \quad \E[v(S)] \quad = \quad \Omega(\E[v(G')]) \quad = \quad \Omega(V^*). \]

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "arxiv"
%%% End: 

